Causal Model Analysis using Collider v-structure with Negative Percentage Mapping

A major problem of causal inference is the arrangement of dependent nodes in a directed acyclic graph (DAG) with path coefficients and observed confounders. Path coefficients do not provide the units to measure the strength of information flowing from one node to the other. Here we proposed the method of causal structure learning using collider v-structures (CVS) with Negative Percentage Mapping (NPM) to get selective thresholds of information strength, to direct the edges and subjective confounders in a DAG. The NPM is used to scale the strength of information passed through nodes in units of percentage from interval from 0 to 1. The causal structures are constructed by bottom up approach using path coefficients, causal directions and confounders, derived implementing collider v-structure and NPM. The method is self-sufficient to observe all the latent confounders present in the causal model and capable of detecting every responsible causal direction. The results are tested for simulated datasets of non-Gaussian distributions and compared with DirectLiNGAM and ICA-LiNGAM to check efficiency of the proposed method.

==> README <==
%%
%% Copyright 1993-2015 LaTeX Project
%%
%% This file is part of the Standard LaTeX `Graphics Bundle'.
%%
%% This file, and all the other files in this bundle as listed below,
%% may be distributed under the terms of the LaTeX Project Public
%% License, as described in lppl.txt in the base LaTeX distribution.
%% Either version 1.3c or, at your option, any later version.
%%
%% The latest version of this license is in
%%
%%   http://www.latex-project.org/lppl.txt
%%
%% and version 1.3c or later is part of all distributions of LaTeX 
%% version 2005/12/01 or later.


The LaTeX Colour and Graphics Packages
========================================
             

This is a collection of LaTeX packages for:
 * producing colour
 * including graphics (eg PostScript) files 
 * rotation and scaling of text
in LaTeX documents.

=======================================================================


THIS DIRECTORY CONTAINS 
======================

README          This File
changes.txt     Log of changes to the packages.
graphics.ins    Install file for docstrip.

Standard packages
=================
color.dtx       Source for color package
graphics.dtx    Source for graphics package
trig.dtx        Source for trig package (required by graphics)

Non Standard Packages
=====================
graphicx.dtx    Source for graphicx package (extension of graphics)
epsfig.dtx      Source for epsfig package (extension of graphicx)
keyval.dtx      Source for keyval pacakge (required by both the above)
lscape.sty      Produce landscape pages in a (mainly) portrait document.

Driver Files
============
drivers.dtx     Source for driver files for supported drivers.

User Documentation
==================
grfguide.tex    User Guide to all the packages in this bundle.
                WARNING: 
                This file calls color and graphics packages
                without a driver option. 
                You *must* set up two files 
                                 color.cfg and graphics.cfg
                containing (for example)
                                \ExecuteOptions{dvips}
                Before running this file.

=============================================

TO UNPACK THE PACKAGES
======================

latex graphics.ins

This will produce the 

.sty package files

Similarly you can run

latex graphics-drivers.ins

to produce the

.def driver files.

Not all supported drivers are included in this file as they are
maintained elsewhere.

=============================================

USING THE PACKAGES
==================

Move files ending in .sty .def  to a standard TeX input directory.

Make a default option for your site by creating two files
     color.cfg and graphics.cfg
containing (if dvips is your default driver)
\ExecuteOptions{dvips}

You may then LaTeX the user guide:
latex grfguide.tex.

==============================================





